Saying Hello World with GReTL - A Solution to the TTC 2011 Instructive Case

This paper discusses the GReTL solution of the TTC 2011 Hello World case. The submitted solution covers all tasks including the optional ones.

==> eptcsdata.tex <==
\providecommand{\firstpage}{295}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.24}{10.4204/EPTCS.74.24}}
\pdfoutput=1

